A Mass-Magnitude Relation for Low-mass Stars Based on Dynamical Measurements of Thousands of Binary Star Systems

Stellar mass is a fundamental parameter that is key to our understanding of stellar formation and evolution, as well as the characterization of nearby exoplanet companions. Historically, stellar masses have been derived from long-term observations of visual or spectroscopic binary star systems. While advances in high-resolution imaging have enabled observations of systems with shorter orbital periods, stellar mass measurements remain challenging, and relatively few have been precisely measured. We present a new statistical approach to measuring masses for populations of stars. Using Gaia astrometry, we analyze the relative orbital motion of $>3,800$ wide binary systems comprising low-mass stars to establish a Mass-Magnitude relation in the Gaia $G_\mathrm{RP}$ band spanning the absolute magnitude range $14.5>M_{G_\mathrm{RP}}>4.0$, corresponding to a mass range of $0.08$~M$_{\odot}\lesssim M\lesssim1.0$~M$_{\odot}$. This relation is directly applicable to $>30$ million stars in the Gaia catalog. Based on comparison to existing Mass-Magnitude relations calibrated for 2MASS $K_{s}$ magnitudes, we estimate that the internal precision of our mass estimates is $\sim$10$\%$. We use this relation to estimate masses for a volume-limited sample of $\sim$18,200 stars within 50~pc of the Sun and the present-day field mass function for stars with $M\lesssim 1.0$~M$_{\odot}$, which we find peaks at 0.16~M$_{\odot}$. We investigate a volume-limited sample of wide binary systems with early K dwarf primaries, complete for binary mass ratios $q>0.2$, and measure the distribution of $q$ at separations $>100$~au. We find that our distribution of $q$ is not uniformly distributed, rather decreasing towards $q=1.0$.

==> hold_text.tex <==
%%$\mu'=\mu/\mu^*$. In terms of measurables, $\mu=\sqrt{\dot{\alpha}^2\cos^2\delta + \dot{\delta}^2}$ and $\mu^*=2\pi\rho^{-1/2}p^{3/2}M_\mathrm{tot}^{1/2}$, with $\rho$, $p$, and $M_\mathrm{tot}$ being the angular separation, parallax, and total mass, respectively. This can be rewritten in absolute quantities as

%\begin{equation}
%\mu' = \frac{\sqrt{s \left( v_\mathrm{x}^2 + %v_\mathrm{y}^2\right)}}{2\pi\sqrt{M_\mathrm{tot}}}.
%\label{eq:muprime_phys}
%\end{equation}

%%Here, we define $s$ as the absolute separation of the components in a binary star system as projected on the sky, and denote $v_\mathrm{x}$ and $v_\mathrm{y}$ as the relative absolute velocities of the secondary star with respect to the primary star. We also adopt the unit system of au-yr-M$_\odot$.

%When transcribed directly into keplerian elements \citep[see, for example][]{Pearce_2020}, $\mu'$ can be described explicitly as a function of the orbit's eccentricity $e$, inclination $i$, argument of periastron $\omega$, and true anomaly $f$, carrying no dependence on the longitude of the ascending node $\Omega$. This allows us to simulate the $\mu'$ distribution for a typical population of binary star systems by first sampling uniformly in $\cos{i}$ from 0 to 1 and in $\omega$ from 0 to 2$\pi$. Then, $f$ is constructed assuming a flat prior from 0 to 2$\pi$ in the mean anomaly and an eccentricity distribution parameterized by $\alpha$ \citep[\textit{see}][]{Hwang2022} as 

%%However, it is also crucial to develop an extended approach to finding masses of stars into the FGK-type regime. \cite{2021AJ....161...36B} found that there could be on average four habitable zone planets around FGK-type stars within $\sim$10~pc of the Sun. It is necessary to derive a method of mass-determination for stars with $M_*>0.70\mathrm{M_\odot}$ to better characterize those planets upon discovery. But making precise masses for individual stars in this range is met with a number of challenges, namely the lack of a better evolutionary model for high-mass stars along the main sequence \citep[\textit{e.g.}][]{1991A&ARv...3...91A, 2010A&ARv..18...67T}.  \textit{...Talk more about the challenges here?..} But 

%Masses of stars in binary systems, for example, can be determined dynamically. Practically, it is only possible to form reliable mass estimates from short-period binaries that are nearby \textbf{(cite?)}. Individual stellar masses can also be directly measured via microlensing, but such observations are infrequent and unpredictable. Thus there exists a strong need for an empirical method for measuring stellar masses, particularly for M dwarfs.

%One popular approach has been to test photometrically-derived mass estimates against those recovered from observations of binary systems. \cite{1993AJ....106..773H} procured a sample of 37 visual binaries with masses dynamically determined to be in the range of $0.08~\mathrm{M}_\odot<M_*<1~\mathrm{M}_\odot$. They observed a mass-luminosity relationship across the $V$-, $J$-, $H$-, and $K$-bandpasses that yielded photometric mass estimates consistent with those measured astrometrically to within $\sim$15\%-20\%. Following this, \cite{2000A&A...364..217D} introduced a mass-luminosity relationship for stars in the range of $0.10~\mathrm{M}_\odot<M_*<0.60~\mathrm{M}_\odot$ good to $\sim$10\%. They showed a decrease in scatter for mass estimates when using near-IR $J$-, $H$-, and $K$-bandpasses. Then, \cite{Benedict_2016} compiled a superset of 47 red dwarfs with $0.08~\mathrm{M}_\odot<M_*<0.62~\mathrm{M}_\odot$ and constructed mass-luminosity relationships in both the $V$- and $K$-bandpasses. They, too, found smaller scatter $\left(\right)$ in the derived mass estimates from the redder $K$-band, particularly for stars with very low mass. The most comprehensive and recent of such analyses was performed by \cite{Mann_2019}, which compared photometrically derived mass estimates to a sample of 62 nearby M dwarf-M dwarf binary systems in the range of $0.075~\mathrm{M}_\odot<M_*<0.70~\mathrm{M}_\odot$, many of which were included in the aforementioned analyses. They used the 2MASS \citep{2006AJ....131.1163S} $K$-short $\left(K_s\right)$ bandpass, which is a truncated version of the Johnson $K$-band. They developed a robust routine for converting 2MASS $K_s$-band magnitudes into reliable mass estimates good to $\sim$1\%-5\% uncertainties.

%The recent evolution of this $M_{K_s}-M_*$ relationship has been administered by an , as well as an increase in the precision of parallaxes, namely from the Gaia mission \citep{2016A&A...595A...1G}. We present a new method


%For an observed population of well-measured binary star systems with a known phase space of on-sky positions and tangent-planes velocities, as well as a distance estimate, the total mass $M_\mathrm{tot}$ is left as the only free parameter needed to determine $\mu'$. We can therefore find the best-fit $M_\mathrm{tot}$ by comparing the simulated $\mu'$ distribution with the observed one. This is described further in Section \ref{sec:LLH}.

% Typical positional and parallax uncertainties in our sample are $\lesssim0.02$~mas for stars with $G\sim7-15$, $\lesssim0.1$~mas for stars with $G\sim15-18$, and $\lesssim1$~mas for stars with $G\gtrsim18$.

%Upon imposing these selection criteria, we are left with XXXX systems, all of which are now vetted for being chance alignments, having poor measurement error, or being of a stellar type not amenable to having its mass estimated via a standard $M-L$ relationship.



(...). Here, we attempt to extend the range of magnitudes for which we are able to make mass estimates. To perform our analysis, we wish to compare the $\mu’$ distribution of our simulated population of binary star systems to our observed sample described in \ref{sec:samp_select}. To do this, we must fit for two free parameters, $\alpha$ and $M_\mathrm{tot}$. By comparing the simulated $\mu'$ distribution to our entire catalog of binary star systems independent of absolute magnitude,   ….mass twin bin stuff….. additionally, \cite{Hwang2021} observed that the eccentricity distribution of binary star systems had a dependence on separation, and since the separation between companions in binaries is correlated to the mass (find cite?), we allow $\alpha$ to float in each bin in such a way that we are jointly fitting for it and $M_\mathrm{tot}$. 

